The moduli space of multi-scale differentials

We construct a compactification of the moduli spaces of abelian differentials on Riemann surfaces with prescribed zeroes and poles. This compactification, called the moduli space of multi-scale differentials, is a complex orbifold with normal crossing boundary. Locally, our compactification can be described as the normalization of an explicit blowup of the incidence variety compactification, which was defined in [BCGGM18] as the closure of the stratum of abelian differentials in the closure of the Hodge bundle. We also define families of projectivized multi-scale differentials, which gives a proper Deligne-Mumford stack, and our compactification is the orbifold corresponding to it. Moreover, we perform a real oriented blowup of the unprojectivized moduli space of multi-scale differentials such that the $\mathrm{GL}_2(\mathbb R)$-action in the interior of the moduli space extends continuously to the boundary.

==> preamble.tex <==
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 %INDEX
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \RequirePackage{filecontents}




\usepackage{tabto}
\usepackage{imakeidx}
\indexsetup{level=\subsection*,toclevel=\paragraph,headers={ \MakeUppercase{Bainbridge, Chen, Gendron, Grushevsky, and M\"oller}}{\MakeUppercase{The moduli space of multi-scale differentials}},noclearpage,firstpagestyle=headings}
\makeindex[name=graph,title=Graphs and Levels,columns=1,columnseprule,options=-s Idx.ist]
\makeindex[name=teich,title=\Teichmuller and Moduli Spaces,columns=1,options=-s Idx.ist]
\makeindex[name=plumb,title=Plumbing Constructions,columns=1,options=-s Idx.ist]
\makeindex[name=twist,title=Prong-matchings and Rotation Groups,columns=1,options=-s Idx.ist]
\makeindex[name=other,title=Other Notations,columns=2,columnseprule,options=-s Idx.ist]
\makeindex[name=surf,title=Surfaces,columns=1,options=-s Idx.ist]
\makeindex[name=family,title=Families,columns=1,options=-s Idx.ist]


% \makeatletter
% \renewcommand*{\@idxitem}{\par \hangindent 2em\hskip 1.5em}% indent the entry
% \makeatother


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Fin index
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\numberwithin{equation}{section}

%% Theorem environments

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lm}[thm]{Lemma}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{add}[thm]{Addendum}
\newtheorem{fact}[thm]{Fact}
\newtheorem{qu}[thm]{Question}
\newtheorem{conj}[thm]{Conjecture}
\newtheorem{summary}[thm]{Summary}
\theoremstyle{definition}
\newtheorem{dfx}[thm]{Definition}
\newenvironment{df}
{\pushQED{\qed}\renewcommand{\qedsymbol}{$\triangle$}\dfx}
{\popQED\enddfx}

\renewcommand{\qedsymbol}{\manimpossiblecube}


\newtheorem{notat}[thm]{Notation}
\newtheorem{rem}[thm]{Remark}
\newtheorem{exa}[thm]{Example}

\newtheorem{ass}{Assumption}


%%%%%%%%%%%%%% equations
\def\={\;=\;}  \def\+{\,+\,} \def\m{\,-\,}
\def\ve{\epsilon}
\def\vare{\varepsilon}
\def\be{\begin{equation}}   \def\ee{\end{equation}}     \def\bes{\begin{equation*}}    \def\ees{\end{equation*}}
\def\ba{\be\begin{aligned}} \def\ea{\end{aligned}\ee}   \def\bas{\bes\begin{aligned}}  \def\eas{\end{aligned}\ees}

%%%%%%%%%%%%%% comments
\definecolor{Mgreen}{RGB}{140,180,0} %
\newcommand{\Dawei}[1]{{\color{red}{Dawei: #1}}}
\newcommand{\Martin}[1]{{\color{Mgreen}{Martin: #1}}}
\newcommand{\Matt}[1]{{\color{cyan}{Matt: #1}}}
\newcommand{\Quentin}[1]{{\color{purple}{Quentin: #1}}}
\newcommand{\Sam}[1]{{\color{blue}{Sam: #1}}}
\newcommand{\Old}[1]{{\color{pink}{Old: #1}}}
\newcommand{\New}[1]{{\color{violet}{#1}}}
\newcommand{\SDM}[1]{{\color{orange}{#1}}}


\newcommand*{\inj}{\hookrightarrow}
\newcommand*{\surj}{\twoheadrightarrow}
\newcommand*{\TC}{\widetilde{C}}
\newcommand*{\TCX}{\widetilde{\calX}}
\newcommand*{\TZ}{\widetilde{Z}}
\newcommand*{\bL}{\overline{L}}
\newcommand*{\bdry}{\partial}
\newcommand*{\ch}{\mbox{ch}}
\newcommand*{\td}{\mbox{td}}
\newcommand*{\wt}{\widetilde}
\newcommand*{\zed}{\mathbb Z}
\newcommand*{\sheafext}{\mathbb{E} \mathrm{xt}}
\newcommand*{\sheafhom}{\mathbb{H} \mathrm{om}}
\newcommand*{\cgeq}{\succcurlyeq}
\newcommand*{\cleq}{\preccurlyeq}
\newcommand*{\tw}{\mathrm{tw}} % Dehn twist

\renewcommand{\tilde}{\widetilde}
\renewcommand{\Re}{\operatorname{Re}}


%math operators

\newcommand*{\Aut}{\operatorname{Aut}}
\newcommand*{\BEff}{\overline{\operatorname{Eff}}}
\newcommand*{\Bl}{\operatorname{Bl}}
\newcommand*{\Blowup}{\operatorname{Bl}}
\newcommand*{\Def}{\operatorname{Def}}
\newcommand*{\Eff}{\operatorname{Eff}}
\newcommand*{\ex}{\operatorname{ex}}
\newcommand*{\Ext}{\operatorname{Ext}}
\newcommand*{\Hom}{\operatorname{Hom}}
\newcommand*{\id}{\operatorname{id}}
\newcommand*{\Jac}{\operatorname{Jac}}
\newcommand*{\lcm}{\operatorname*{lcm}}
\newcommand*{\Obs}{\operatorname{Obs}}
\newcommand*{\PGL}{\operatorname{PGL}}
\newcommand*{\Pic}{\operatorname{Pic}}
%\newcommand*{\Pl}{\operatorname{Pl}}
\newcommand*{\QC}{\operatorname{QC}}
\newcommand*{\OuPl}{\Omega\operatorname{uPl}}
\newcommand*{\uPl}{\operatorname{uPl}}
\newcommand*{\OPl}{\Omega\operatorname{Pl}}
\newcommand*{\OPlv}{\Omega\operatorname{Pl}^v}
%\newcommand*{\OPlh}{\Omega\operatorname{Pl^h}}
\newcommand*{\Res}{\operatorname{Res}}
\newcommand*{\SL}{\mathrm{SL}}
\newcommand*{\GL}{\mathrm{GL}}
\newcommand*{\Spec}{\operatorname{Spec}}
\newcommand*{\Supp}{\operatorname{Supp}}
\newcommand*{\chern}{\operatorname{ch}}
\newcommand*{\ct}{\operatorname{ct}}
\newcommand*{\eff}{\operatorname{eff}}
\newcommand*{\even}{\operatorname{even}}
\newcommand*{\hyp}{\operatorname{hyp}}
\newcommand*{\alg}{\operatorname{alg}}
\newcommand*{\an}{\operatorname{an}}
\newcommand*{\irr}{\operatorname{irr}}
\newcommand*{\nh}{\operatorname{non-hyp}}
\newcommand*{\nonhyp}{\operatorname{non-hyp}}
\newcommand*{\nonws}{\operatorname{non-ws}}
\newcommand*{\odd}{\operatorname{odd}}
\newcommand*{\ord}{\operatorname{ord}}
\newcommand*{\other}{\operatorname{other}}
\newcommand*{\Proj}{\operatorname{Proj}}
\newcommand*{\rank}{\operatorname{rank}}
\newcommand*{\red}{\operatorname{red}}
\newcommand*{\reg}{\operatorname{reg}}
\newcommand*{\sm}{\operatorname{sm}}
\newcommand*{\topo}{\operatorname{top}}
\newcommand*{\ws}{\operatorname{ws}}

\newcommand*{\germs}[1][\mathcal{X}/B]{\mathcal{E}_{#1}}


\newcommand*{\eq}{{\rm eq}}



\newcommand{\dualgraph}{\Gamma_{\rm dual}}
\newcommand{\dualgraphspe}{\Gamma_{p}}
\newcommand{\dualgraphgen}{\Gamma_{{\rm dual}}^{\rm gen}}
\newcommand{\dualsheave}[1][X]{\omega_{#1}}
\newcommand{\holoneform}[1][X]{\Omega_{#1}^{1}}
\newcommand{\turn}{\operatorname{tu}}
\newcommand{\Weld}{\operatorname{Weld}}
\newcommand{\Span}{\operatorname{span}}
\renewcommand{\Pr}{{\rm Pr}}

\newcommand{\Gammagen}[1][p]{\Gamma^\mathrm{gen}_{#1}}
\newcommand{\Lambdagen}[1][p]{\Lambda^\mathrm{gen}_{#1}}

\newcommand{\divisor}[1]{{\rm div }\left( #1 \right)}
\newcommand{\divzero}[1]{{\rm div }_{0}\left( #1 \right)}
\newcommand{\banach}[2]{\calO(#1)_{#2}}
\newcommand{\permGroup}[1][n]{\mathfrak{S}_{#1}}
\newcommand{\isom}{\cong}
\newcommand{\rom}[1]{\textup{\uppercase\expandafter{\romannumeral#1}}}
\newcommand{\op}{\operatorname}
\newcommand{\val}{\op{val}}

\newcommand{\ver}{{v}}
\newcommand{\hor}{{h}}
\newcommand{\Per}{{\rm Per}}
\newcommand{\PPer}{{\rm PPer}}
\newcommand{\ePP}{{\rm ePP}}
\newcommand{\Phor}{{\rm Phor}}

\newcommand{\del}{\partial}
\newcommand{\delbar}{\bar{\partial}}
\newcommand*{\degen}{{\rm dg}}
\newcommand*{\degenbar}{\overline{{\rm dg}}}


\newcommand{\ol}{\overline}
\newcommand{\ul}{\underline}


%names

\newcommand*{\Mobius}{M\"obius\xspace}
\newcommand*{\Poincare}{Poincar\'e\xspace}
\newcommand*{\Holder}{H\"older\xspace}
\newcommand*{\Teichmuller}{Teich\-m\"uller\xspace}
\newcommand*{\Bezout}{B\'ezout\xspace}
\newcommand*{\Caratheodory}{Carath\'eodory\xspace}

\newcommand*{\etale}{\'etale\xspace}
\newcommand*{\espaceetale}{\'etal\'e space\xspace}

%caligraphic

\newcommand*{\calA}{\mathcal A}
\newcommand*{\calB}{\mathcal B}
\newcommand*{\calC}{\mathcal C}
\newcommand*{\calD}{\mathcal D}
\newcommand*{\calE}{\mathcal E}
\newcommand*{\calF}{\mathcal F}
\newcommand*{\calG}{\mathcal G}
\newcommand*{\calH}{\mathcal H}
\newcommand*{\calI}{\mathcal I}
\newcommand*{\calJ}{\mathcal J}
\newcommand*{\calL}{\mathcal L}
\newcommand{\calM}{{\mathcal M}}
\newcommand{\calO}{{\mathcal O}}
\newcommand*{\calP}{\mathcal P}
\newcommand{\calQ}{{\mathcal Q}}
\newcommand{\calN}{{\mathcal N}}
\newcommand*{\calR}{\mathcal R}
\newcommand*{\calS}{\mathcal S}
\newcommand{\calT}{{\mathcal T}}
\newcommand{\calU}{{\mathcal U}}
\newcommand{\calV}{{\mathcal V}}
\newcommand*{\calX}{\mathcal X}
\newcommand{\calW}{\mathcal W}
\newcommand{\calZ}{{\mathcal Z}}
\newcommand{\bfcalZ}{{\boldsymbol{\mathcal Z}}}
\newcommand{\calY}{{\mathcal Y}}

\newcommand{\mfm}{{\mathfrak m}}

%boldsymbols
\newcommand{\CC}{{\mathbb{C}}}
\renewcommand{\AA}{{\mathbb{A}}}
\newcommand{\GG}{{\mathbb{G}}}
\newcommand{\HH}{{\mathbb{H}}}
\newcommand{\FF}{{\mathbb{F}}}
\newcommand{\WW}{{\mathbb{W}}}
\newcommand{\EE}{{\mathbb{E}}}
\newcommand{\PP}{{\mathbb{P}}}
\newcommand{\QQ}{{\mathbb{Q}}}
\newcommand{\RR}{{\mathbb{R}}}
\newcommand{\ZZ}{{\mathbb{Z}}}
\newcommand{\MM}{{\mathbb{M}}}
\newcommand{\NN}{{\mathbb{N}}}
\newcommand{\DD}{{\mathbb{D}}}
\newcommand{\VV}{{\mathbb{V}}}
% alternative bold letter commands
\newcommand*{\ratls}{\mathbb{Q}}
\newcommand*{\reals}{\mathbb{R}}
\newcommand*{\cx}{\mathbb{C}}
\newcommand*{\nats}{\mathbb{N}}
\newcommand*{\proj}{\mathbb{P}}
\newcommand*{\half}{\mathbb{H}}


% boldletters
\newcommand*{\kk}{{\boldsymbol\kappa}}
\newcommand{\bfa}{{\boldsymbol{a}}}
\newcommand{\bfb}{{\boldsymbol{b}}}
\newcommand{\bfc}{{\boldsymbol{c}}}
\newcommand{\bfd}{{\boldsymbol{d}}}
\newcommand{\bfe}{{\boldsymbol{e}}}
\newcommand{\bfE}{{\boldsymbol{E}}}
\newcommand{\bff}{{\boldsymbol{f}}}
\newcommand{\bfm}{{\boldsymbol{m}}}
\newcommand{\bfmu}{{\boldsymbol{\mu}}}
\newcommand{\bfn}{{\boldsymbol{n}}}
\newcommand{\bfp}{{\boldsymbol{p}}}
\newcommand{\bfq}{{\boldsymbol{q}}}
\newcommand{\bfR}{{\boldsymbol{R}}}
\newcommand{\bfU}{{\boldsymbol{U}}}
\newcommand{\bfu}{{\boldsymbol{u}}}
\newcommand{\bfw}{{\boldsymbol{w}}}
\newcommand{\bfy}{{\boldsymbol{y}}}
\newcommand{\bfx}{{\boldsymbol{x}}}
\newcommand{\bfs}{{\boldsymbol{s}}}
\newcommand{\bfS}{{\boldsymbol{S}}}
\newcommand{\bfT}{{\boldsymbol{T}}}
\newcommand{\bft}{{\boldsymbol{t}}}
\newcommand{\bfz}{{\boldsymbol{z}}}
\newcommand{\bfsigma}{{\boldsymbol{\sigma}}}
\newcommand{\bftau}{{\boldsymbol{\tau}}}
%\newcommand{\bftheta}{{\boldsymbol{\theta}}}
\newcommand{\bfeta}{{\boldsymbol{\eta}}}
\newcommand{\bfomega}{{\boldsymbol{\omega}}}
\newcommand{\bfxi}{{\boldsymbol{\xi}}}
\newcommand{\bfzero}{{\boldsymbol{0}}}
%underlines

\newcommand*\us{{\underline{s}}}
\newcommand*\uu{{\underline{u}}}
\newcommand*\uv{{\underline{v}}}
\newcommand*\uw{{\underline{w}}}
\newcommand*\ut{{\underline{t}}}
\newcommand*\uz{{\underline{z}}}
\newcommand*\um{{\underline{m}}}
\newcommand*\uM{{\underline{M}}}
\newcommand*\uR{{\underline{R}}}
\newcommand*\ur{{\underline{r}}}
\newcommand*\uk{{\underline{k}}}
\newcommand*\un{{\underline{n}}}
\newcommand*\uN{{\underline{N}}}

%overlines
\newcommand*\on{{\overline{n}}}

%tildes
\newcommand{\tu}{\widetilde{u}}
\newcommand{\tv}{\widetilde{v}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%abbreviations

% MODULI SPACES
% abelian varieties
%\newcommand{\AVmoduli}[1][g]{{\mathcal A}_{#1}}
%\newcommand{\oAVmoduli}[1][g]{{\Omega\mathcal A}_{#1}}
% curves
% notations we always had consensus on / IVC-compactification notation
\newcommand{\barmoduli}[1][g]{{\overline{\mathcal M}}_{#1}}
\newcommand{\moduli}[1][g]{{\mathcal M}_{#1}}
\newcommand{\omoduli}[1][g]{{\Omega\mathcal M}_{#1}}
\newcommand{\modulin}[1][g,n]{{\mathcal M}_{#1}}
\newcommand{\omodulin}[1][g,n]{{\Omega\mathcal M}_{#1}}
\newcommand{\zomoduli}[1][]{{\mathcal H}_{#1}}
\newcommand{\barzomoduli}[1][]{{\overline{\mathcal H}_{#1}}}
\newcommand{\pomoduli}[1][g]{{\proj\Omega\mathcal M}_{#1}}
\newcommand{\pomodulin}[1][g,n]{{\proj\Omega\mathcal M}_{#1}}
\newcommand{\pobarmoduli}[1][g]{{\proj\Omega\overline{\mathcal M}}_{#1}}
\newcommand{\pobarmodulin}[1][g,n]{{\proj\Omega\overline{\mathcal M}}_{#1}}
\newcommand{\potmoduli}[1][g]{\proj\Omega\tilde{\mathcal{M}}_{#1}}
\newcommand{\obarmoduli}[1][g]{{\Omega\overline{\mathcal M}}_{#1}}
\newcommand{\obarmodulio}[1][g]{{\Omega\overline{\mathcal M}}_{#1}^{0}}
\newcommand{\otmoduli}[1][g]{\Omega\tilde{\mathcal{M}}_{#1}}
\newcommand{\pom}[1][g]{\proj\Omega{\mathcal M}_{#1}}
\newcommand{\pobarm}[1][g]{\proj\Omega\overline{\mathcal M}_{#1}}
\newcommand{\pobarmn}[1][g,n]{\proj\Omega\overline{\mathcal M}_{#1}}
\newcommand{\princbound}{\partial\mathcal{H}}
\newcommand{\omoduliinc}[2][g,n]{{\Omega\mathcal M}_{#1}^{{\rm inc}}(#2)}
\newcommand{\obarmoduliinc}[2][g,n]{{\Omega\overline{\mathcal M}}_{#1}^{{\rm inc}}(#2)}
\newcommand{\pobarmoduliinc}[2][g,n]{{\proj\Omega\overline{\mathcal M}}_{#1}^{{\rm inc}}(#2)}
\newcommand{\otildemoduliinc}[2][g,n]{{\Omega\widetilde{\mathcal M}}_{#1}^{{\rm inc}}(#2)}
\newcommand{\potildemoduliinc}[2][g,n]{{\proj\Omega\widetilde{\mathcal M}}_{#1}^{{\rm inc}}(#2)}
\newcommand{\omoduliincp}[2][g,\lbrace n \rbrace]{{\Omega\mathcal M}_{#1}^{{\rm inc}}(#2)}
\newcommand{\obarmoduliincp}[2][g,\lbrace n \rbrace]{{\Omega\overline{\mathcal M}}_{#1}^{{\rm inc}}(#2)}
\newcommand{\obarmodulin}[1][g,n]{{\Omega\overline{\mathcal M}}_{#1}}
\newcommand{\N}[1][X]{N_{#1}} %nodes of #1
\newcommand{\Nver}[1][X]{N_{#1}^{\ver}} %nodes of #1
\newcommand{\Nhor}[1][X]{N_{#1}^{\hor}} %nodes of #1
\newcommand{\SLtwoR}{\SL_2(\reals)}
\newcommand{\GLtwoRplus}{\GL_2^+(\reals)}


%%%Teichmuller spaces
\DeclareDocumentCommand{\teich}{ O{\Sigma} O{\bfs}}{{\mathcal T}_{(#1,#2)}}
\newcommand{\oldteich}[1][g,n]{{\mathcal T}_{#1}}
\DeclareDocumentCommand{\Pteich}{ O{\Sigma} O{\bfs} O{\mu}}{\mathcal{T}_{(#1,#2)}(#3)}
\DeclareDocumentCommand{\bigPteich}{ O{\Sigma} O{\bfs} O{\mu}}{\mathcal{T}^+_{(#1,#2)}(#3)}
\DeclareDocumentCommand{\Oteich}{ O{\Sigma} O{\bfs} O{\mu}}{\Omega \mathcal{T}_{(#1,#2)}(#3)}
\DeclareDocumentCommand{\bigOteich}{ O{\Sigma} O{\bfs} O{\mu}}{\Omega\mathcal{T}^+_{(#1,#2)}(#3)}
\DeclareDocumentCommand{\augteich}{ O{\Sigma} O{\bfs}}{{\overline{\mathcal T}}_{(#1,#2)}}
\newcommand{\oldaugteich}[1][g,n]{{\overline{\mathcal T}}_{#1}}
\newcommand{\famaugteich}[1][g,n]{\overline{\calX}_{#1}}
\DeclareDocumentCommand{\BSteich}{ O{\Sigma} O{\bfs}}{{\overline{\mathcal T}}^{\rm BS}_{(#1,#2)}}
\DeclareDocumentCommand{\Bteich}{ O{\Lambda} }{{{\mathcal T}}_{#1}}
\DeclareDocumentCommand{\BBSteich}{ O{\Lambda} }{{{\mathcal T}}^{\rm BS}_{#1}}
\DeclareDocumentCommand{\BBBSteich}{ O{\Lambda} }{{\widehat{{\mathcal T}}}^{\rm BS}_{#1}}
\DeclareDocumentCommand{\BPteich}{ O{\Lambda} O{\mu}}{\mathcal{T}_{#1}(#2)}
\DeclareDocumentCommand{\OBnoGRC}{ O{\Lambda} O{\mu}}{\Omega^{no} {{\mathcal T}}_{#1}(#2)}
\DeclareDocumentCommand{\OBteich}{ O{\Lambda} O{\mu}}{\Omega {{\mathcal T}}_{#1}(#2)}
\DeclareDocumentCommand{\OBBSteich}{ O{\Lambda} O{\mu}}{\Omega{{\mathcal T}}^{\rm BS}_{#1}(#2)}

%\newcommand*{\ptwT}[1][\Lambda] {{\Omega\mathcal{T}^{pm}_{#1}}}




%%% Mapping class groups
%\DeclareDocumentCommand{\Mod}{ O{\Sigma} O{\bfs}}{\operatorname{Mod}_{(#1,#2)}}
\newcommand{\Mod}[1][g,n]{\operatorname{Mod}_{#1}}
\DeclareDocumentCommand{\flatMod}{ O{\Sigma} O{\bfs} O{\mu}}{\operatorname{Mod}_{(#1,#2)}(\mu)}
\DeclareDocumentCommand{\TNP}{ O{\Sigma} O{\bfs} O{\mu}}{\operatorname{TNP}_{(#1,#2)}(\mu)}
% \newcommand{\oldMod}[1][g,n]{\operatorname{Mod}_{#1}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% Graphs with decoration

\newcommand{\aG}{\Gamma}                  % abstract graph
\newcommand{\dG}{\Gamma_{X}}                  % standard dual graph
\newcommand{\lG}{\Gamma}     % level graph (i.e. with level structure)
\newcommand{\lGp}{{\overline{\Gamma}}}     % level graph (i.e. with level structure)
\newcommand{\eG}{\Gamma}       % enhanced level graph
\newcommand{\eGp}{\Gamma^{+}}     % enhanced level graph
\newcommand{\oL}{{\overline{\Lambda}}}              % ordered multicurve
\newcommand{\eL}{\Lambda}                   % enhanced multicurve
\newcommand{\eLp}{\Lambda^{+}}                   % enhanced multicurve
\newcommand{\ltop}[1][e]{\ell(#1^{+})}                   % Top level of a node
\newcommand{\lbot}[1][e]{\ell(#1^{-})}                  % Bottom level of a node
\newcommand{\lqtop}[1][q]{\ell(#1^{+})}                   % Level of the top point of a node
\newcommand{\lqbot}[1][q]{\ell(#1^{-})}                  %  Level of the bottom point of a node
\newcommand{\ltopbot}[1][e]{\ell(#1^{\pm})}                  % Bottom and top level of a node
\newcommand{\lqtopbot}[1][q]{\ell(#1^{\pm})}                   % Level of the top and bottom points of a node
\newcommand{\topvert}[1][e]{#1^{+}}   % top vertex of an edge
\newcommand{\botvert}[1][e]{#1^{-}}  % bottom vertex of an edge
\newcommand{\topbotvert}[1][e]{#1^{\pm}}   % top  and bottom vertex of an edge

\newcommand{\horedge}[1][\lG]{E(#1)^{\hor}}   % horizontal edges
\newcommand{\vertedge}[1][\lG]{E(#1)^{\ver}}  % vertical edges

\newcommand{\prodt}[1][\lceil i \rceil]{\bft^\bfa_{#1}}
\newcommand{\prods}[1][\lceil i \rceil]{s_{#1}}
\newcommand{\prodttop}[1][\lceil \ltop\rceil]{\bft^\bfa_{#1}}
\newcommand{\prodtbot}[1][\lceil \lbot\rceil]{\bft^\bfa_{#1}}
\newcommand{\prodthor}[1][\lceil \ell(h)\rceil]{\bft^\bfa_{#1}}

\DeclareDocumentCommand{\pin}{ O{z} O{\omega}}{P^{\rm in}_{#1}}
\DeclareDocumentCommand{\pout}{ O{z} O{\omega}}{P^{\rm out}_{#1}}
%prongs with angles
% \DeclareDocumentCommand{\pin}{ O{z,\theta} O{\omega}}{P^{\rm in}_{#1}(#2)}
% \DeclareDocumentCommand{\pout}{ O{z,\theta} O{\omega}}{P^{\rm out}_{#1}(#2)}

%g%% Level rotation tori and Twist groups
\newcommand*{\Prot}[1][\eG]{{P_{#1}}}
% Prong rotation group (of card \prod_{all} (k_i +1))
\newcommand*{\Ttwd}[1][\eG]{T^\mathrm{tw}_{#1}}
\newcommand*{\Tprong}[1][\eG]{T_{#1}}
\newcommand*{\Tred}[1][\Lambda]{T^{0}_{#1}}
\newcommand*{\Textd}[1][\Lambda]{T^{\bullet}_{#1}}
\newcommand*{\Tsimp}[1][\Lambda]{T^s_{#1}}
\newcommand*{\Tsred}[1][\Lambda]{T^{s,0}_{#1}}
\newcommand*{\Tsextd}[1][\Lambda]{T^{s,\bullet}_{#1}}
\newcommand*{\Ttorsor}[1][\eG]{\mathfrak{T}_{#1}}
\newcommand*{\Tstorsor}[1][\eG]{\mathfrak{T}^s_{#1}}
\newcommand*{\Tmtorsor}[1][\eG]{\mathfrak{T}^m_{#1}}
\newcommand*{\Tmstorsor}[1][\eG]{\mathfrak{T}^{ms}_{#1}}


\newcommand*{\Tnorm}[1][\Lambda]{\overline{T}_{#1}^{n}}
\newcommand*{\Tsnorm}[1][\Lambda]{\overline{T}_{#1}^{s}}


\newcommand*{\Tmulti}[1][\Lambda]{{\widetilde{T}_{#1}}}
\newcommand*{\Tprongz}[1][\eG]{T_{#1}^0} % all but top level
\newcommand*{\Tmultiz}[1][\Lambda]{{\widetilde{T}_{#1}^0}}  % all but top level

\newcommand*{\Tw}[1][\Lambda]{\mathrm{Tw}_{#1}}  %twist group
\newcommand*{\sTw}[1][\Lambda]{\mathrm{Tw}_{#1}^s}  %simple twist group
\DeclareDocumentCommand{\sTwi}{ O{\Lambda} O{i}}{\mathrm{Tw}_{#1,#2}^{sv}}  %ith simple twist group
\newcommand*{\vTw}[1][\Lambda]{\mathrm{Tw}_{#1}^v}  %vertical twist group
\newcommand*{\svTw}[1][\Lambda]{\mathrm{Tw}_{#1}^{sv}}  %simple vertical twist group
\newcommand*{\hTw}[1][\Lambda]{\mathrm{Tw}_{#1}^h}  %horizontal twist group
\newcommand*{\shTw}[1][\Lambda]{\mathrm{Tw}_{#1}^{sh}}  %simple horizontal twist group

\newcommand*{\oldtwist}[1][\Lambda]{\mathrm{Tw}_{#1}^{\rm full}}
\newcommand*{\rottwist}[1][\Lambda]{\mathrm{Tw}_{#1}^{\rm rot}}

%classical twist group (requires no notion/definion of levels)


%%%%%%%%%%%%%%%
\newcommand{\twd}{twisted differential\xspace}
\newcommand{\twds}{twisted\ differentials\xspace}
\newcommand*{\ptwd}{prong-matched twisted differential\xspace}
\newcommand*{\ptwds}{prong-matched twisted differentials\xspace}
\newcommand*{\Ptwds}{Prong-matched twisted differentials\xspace}
\newcommand*{\mptwd}{marked prong-matched twisted differential\xspace}
\newcommand*{\mptwds}{marked prong-matched twisted differentials\xspace}

\newcommand*{\msd}{multi-scale differential\xspace}
\newcommand*{\tnp}{turning-number-preserving\xspace}
\newcommand*{\prma}{prong-matching\xspace}
\newcommand*{\Prma}{Prong-matching\xspace}
\newcommand*{\prmas}{prong-matchings\xspace}
\newcommand*{\Prmas}{Prong-matchings\xspace}
\newcommand*{\Msd}{Multi-scale differential\xspace}
\newcommand*{\msds}{multi-scale differentials\xspace}
\newcommand*{\Msds}{Multi-scale differentials\xspace}
\newcommand*{\auxd}{model differential\xspace}
\newcommand*{\auxds}{model differentials\xspace}
\newcommand*{\lw}{level-wise\xspace}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Corresponding moduli space of differentials
\newcommand*{\twM}[1][\eG]{{\Omega\mathcal{M}^{{\rm tw}}_{#1}}}
\newcommand*{\ptwM}[1][\eG] {{\Omega\mathcal{M}^p_{#1}}}
% this an unramified P_\oG-cover of \oM (P_\oG = prong group)
% corresponding partial compactifications (for defining plumbing map)
\newcommand*{\bartwM}[1][\eG]{{\overline{\Omega\mathcal{M}}^{{\rm tw}}_{#1}}}
\newcommand*{\barptwM}[1][\eG] {{\overline{\Omega\mathcal{M}}^p_{#1}}}

\DeclareDocumentCommand{\kmoduli}{ O{\mu} O{g} O{n} }{\mathcal{M}_{#2,#3}(#1)}
\DeclareDocumentCommand{\barkmoduli}{ O{\mu} O{g} O{n} }{\mathcal{\overline{M}}_{#2,#3}(#1)}
\DeclareDocumentCommand{\obarkmoduli}{ O{\mu} O{g} O{n} }{\Omega\mathcal{\overline{M}}_{#2,#3}(#1)}


\DeclareDocumentCommand{\LMS}{ O{\mu} O{g,n}} {\Xi\overline{\mathcal{M}}_{#2}(#1)}
\DeclareDocumentCommand{\RBLMS}{ O{\mu} O{g,n}}
%OLD                       {\widehat{\Xi\overline{\mathcal{M}}}_{#2}(#1)}
{\Xi\widehat{\mathcal{M}}_{#2}(#1)}




% scaled version of these spaces, modulo the tori
\newcommand*{\msT}[1][\Lambda]{{\Omega\calB_{#1}}}
\newcommand*{\pmsT}[1][\Lambda]{\proj \Omega \calB_{#1}}

\newcommand*{\kmsT}[1][\Lambda]{{\Omega^{k}\calB_{#1}}}

\newcommand*{\MD}[1][\Lambda]{{\mathcal MD}_{#1}} %The model domain
\newcommand*{\OMD}[1][\Lambda]{\Omega{\mathcal MD}_{#1}} %The model domain
\newcommand*{\barMD}[1][\Lambda]{\overline{{\mathcal MD}}_{#1}} %Its closure
\newcommand*{\barOMD}[1][\Lambda]{\Omega\overline{{\mathcal MD}}_{#1}} %Its closure
\DeclareDocumentCommand{\MDstratum}{ O{\Lambda} O{\Lambda'}}{\mathcal{MD}_{#1}^{#2}}
\DeclareDocumentCommand{\OMDstratum}{  O{\Lambda} O{\Lambda'}}{\Omega\mathcal{MD}_{#1}^{#2}}
\newcommand*{\MDs}[1][\Lambda]{{\mathcal MD}^s_{#1}}
%The model domain: simple version
\newcommand*{\barMDs}[1][\Lambda]{\overline{{\mathcal MD}}^s_{#1}} %Its closure
\newcommand*{\barOMDs}[1][\Lambda]{\Omega\overline{{\mathcal MD}}^s_{#1}} %Its closure
\DeclareDocumentCommand{\MDstratums}{ O{\Lambda} O{\Lambda'}}{\mathcal{MD}_{#1}^{s,#2}}


\newcommand*{\PD}[1][\Lambda]{{\mathcal PD}_{#1}} %The Plumbing domain
\newcommand*{\barPD}[1][\Lambda]{\overline{{\mathcal PD}}_{#1}} %Its closure
\DeclareDocumentCommand{\PDstratum}{ O{\Lambda} O{\Lambda'}}{\mathcal{PD}_{#1}^{#2}}


% marked prong-matched (i.e. Teichmueller spaces)
\newcommand*{\barptwT}[1][\Lambda] {{\overline{\Omega\mathcal{T}}^p_{#1}}}
\DeclareDocumentCommand{\ptwT}{ O{\Lambda} O{\mu}}{{\Omega\mathcal{T}^{pm}_{#1}(#2)}}
\DeclareDocumentCommand{\ptwTm}{ O{\Lambda} O{\mu}}{{\Omega\mathcal{T}^{pm}_{#1}(#2)^-}}

\DeclareDocumentCommand{\kptwT}{ O{\Lambda} O{\mu}}{{\Omega^{k}\mathcal{T}^{pm}_{#1}(#2)}}

% total spaces

\DeclareDocumentCommand{\ocpM}{ O{g} O{\mu}}{\Omega{\overline{\mathcal{M}}_{#1}({#2})}}
% "compactification" of \Omega M_g(\mu)

\DeclareDocumentCommand{\cpM}{ O{g} O{\mu}}{{\overline{\mathcal{M}}_{#1}({#2})}}  %compactification
% of \Omega M_g,n(\mu) / C^*

\DeclareDocumentCommand{\Oaugteich}{ O{\Sigma} O{\bfs} O{\mu}}{\Omega \overline{\mathcal{T}}_{(#1,#2)}(#3)}
\DeclareDocumentCommand{\Okaugteich}{ O{\Sigma} O{\bfs} O{\mu}}{\Omega^{k} \overline{\mathcal{T}}_{(#1,#2)}(#3)}
%Aug. Teich. space of flat surfaces

\DeclareDocumentCommand{\Paugteich}{ O{\Sigma} O{\bfs} O{\mu}}{\PP \Omega \overline{\mathcal{T}}_{(#1,#2)}(#3)} %Augmented Teich. space of canonical divisors

%Mapping Class Group
\newcommand*{\MCG}[1][\Sigma, \xi]{\mathrm{Mod}(#1)}

% Dehn  space version
\newcommand*{\Dehn[1]}[\Lambda]{{\PP\Xi\mathcal{D}_{#1}}}
\newcommand*{\Dehns[1]}[\Lambda]{{\PP\Xi\mathcal{D}^s_{#1}}}
\newcommand*{\ODehn[1]}[\Lambda]{{\Xi\mathcal{D}_{#1}}}
\newcommand*{\ODehns[1]}[\Lambda]{{\Xi\mathcal{D}^s_{#1}}}
\newcommand*{\ODehnsv[1]}[\Lambda]{{\Xi\mathcal{D}^{sv}_{#1}}}
%% OBSOLETE\newcommand*{\Dehnorb[1]}[\Lambda]{{\mathcal{D}^{\rm orb}_{#1}}}
\DeclareDocumentCommand{\Dstratum}{ O{\Lambda} O{\Lambda'}}{{\PP\Xi\mathcal D}_#1^{#2}}
\DeclareDocumentCommand{\Dstratums}{ O{\Lambda} O{\Lambda'}}{{\PP\Xi\mathcal D}_#1^{#2,s}}
\DeclareDocumentCommand{\ODstratum}{ O{\Lambda} O{\Lambda'}}{{\Xi\mathcal D}_#1^{#2}}
\DeclareDocumentCommand{\ODstratums}{ O{\Lambda} O{\Lambda'}}{{\Xi\mathcal D}_#1^{#2,s}}
\DeclareDocumentCommand{\ODstratumso}{ O{\Lambda} O{\Lambda'}}{{\Xi\mathcal D}_{#1,\circ}^{#2,s}}
\DeclareDocumentCommand{\ODstratumo}{ O{\Lambda} O{\Lambda'}}{{\Xi\mathcal D}_{#1,\circ}^{#2}}

%%% OBSOLETE \DeclareDocumentCommand{\Dorbstratum}{ O{\Lambda} O{\Lambda'}}{{\mathcal D}_#1^{{\rm orb},#2}}

\newcommand{\oldDehn}[1][\Lambda]{\mathcal{D}_{#1}}
\newcommand{\ooldDehn}[1][\Lambda]{\Omega\mathcal{D}_{#1}}
\newcommand*{\oldDehnfam}[1][\Lambda]{\calX_{#1}}

%families over Dehn space
\newcommand*{\Dehnfam[1]}[\Lambda]{{\calX_{#1}}}
\newcommand*{\Dehnsfam[1]}[\Lambda]{{\calX^s_{#1}}}
\newcommand*{\ODehnfam[1]}[\Lambda]{{\Omega\calX_{#1}}}
\newcommand*{\ODehnsfam[1]}[\Lambda]{{\Omega\calX^s_{#1}}}

%families over the model domain
\newcommand*{\MDfam[1]}[\Lambda]{{\calX}}
\newcommand*{\MDsfam[1]}[\Lambda]{{\calX}}
\newcommand*{\OMDfam[1]}[\Lambda]{{\calX}}
\newcommand*{\OMDsfam[1]}[\Lambda]{{\calX}}

%universal family
\newcommand*{\unifam}{{\calX}}
\newcommand*{\barunifam}{{\ol{\calX}}}


%Functors
\DeclareDocumentCommand{\sMSfmark}{ O{\mu} O{\eL}}{\mathbf{MS}^s_{(#1,#2)}}
\DeclareDocumentCommand{\MSfmark}{ O{\mu} O{\eL}}{\mathbf{MS}_{(#1,#2)}}
\DeclareDocumentCommand{\sMSfun}{ O{\mu} }{\mathbf{MS}^s_{#1}}
\DeclareDocumentCommand{\MSfun}{ O{\mu} }{\mathbf{MS}_{#1}}
%% THIS ONE HAS NEITHER GAMMA NOR LAMBDA!!!
\DeclareDocumentCommand{\MSgrp}{ O{\mu} }{\mathcal{MS}_{#1}}

\DeclareDocumentCommand{\sMDfmark}{ O{\mu} O{\eL}}{\mathbf{MD}^s_{(#1,#2)}}
\DeclareDocumentCommand{\MDfmark}{ O{\mu} O{\eL}}{\mathbf{MD}_{(#1,#2)}}
\DeclareDocumentCommand{\MDfun}{ O{\mu} O{\eG}}{\mathbf{MD}_{(#1,#2)}}


%generalised diffeo and nearly smooth surfaces.
\newcommand*{\diffeogen}{almost-diffeomorphism\xspace}
\newcommand*{\diffeogens}{almost-diffeomorphisms\xspace}

\newcommand*{\nearsm}{almost smooth surface\xspace}
\newcommand*{\nearsms}{almost smooth surfaces\xspace}











%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%New Commands for k-Diff!!!!
\newcommand{\Ox}[1][X]{\calO_{#1}}
\newcommand{\im}{{\rm Im}}
\newcommand{\whX}{\widehat{X}}
\newcommand{\whY}{\widehat{Y}}
\newcommand{\whP}{\widehat{P}}
\newcommand{\whZ}{\widehat{Z}}
\newcommand{\whz}{\widehat{z}}
\newcommand{\whg}{\widehat{g}}
\newcommand{\whmu}{\widehat{\mu}}
\newcommand{\whLa}{\widehat{\Lambda}}
\newcommand{\whq}{\widehat{q}}
\newcommand{\whsigma}{\widehat{\sigma}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\divomega}{D}
\newcommand{\divomegared}{D_{\rm red}}
\newcommand{\divxi}{E}
\newcommand{\divxired}{E_{\rm red}}
\newcommand{\komoduli}[1][g]{{\Omega^k\mathcal M}_{#1}}
\newcommand{\komoduliab}[1][\mu]{\Omega^{k,{\operatorname{ab}}}\mathcal{M}_{g}(#1)}
\newcommand{\komodulinoab}[1][\mu]{\Omega^{k,{\operatorname{non-ab}}}\mathcal{M}_{g}(#1)}
\newcommand{\tkdab}[1][\overline{\Gamma}]{\mathfrak{W}^{k, \operatorname{ab}}(#1)}
\newcommand{\tkdnoab}[1][\overline{\Gamma}]{\mathfrak{W}^{k, \operatorname{non-ab}}(#1)}
\newcommand{\tdab}[1][\overline{\Gamma}]{\mathfrak{W}^{\operatorname{ab}}(#1)}

\newcommand{\komodulin}[1][g,n]{{\Omega^k\mathcal M}_{#1}}
\newcommand{\kobarmoduli}[1][g]{{\Omega^k\overline{\mathcal M}}_{#1}}
\newcommand{\kobarmodulin}[1][g,n]{{\Omega^k\overline{\mathcal M}}_{#1}}
\newcommand{\kivc}[2][g,n]{{\PP\Omega^k{\overline{\mathcal M}}_{#1}^{{\rm inc}}(#2)}}
\newcommand{\Resk}[1][k]{\Res^{#1}}
\newcommand{\cplxlie}{\mathcal{C}^{\bullet}(\Lied[\omega])}
\newcommand{\cplxliek}{\mathcal{C}^{\bullet}(\Lied)}
\newcommand{\Lied}[1][\xi]{\mathcal{L}_{#1}}
\newcommand{\whomega}{\wh\omega}
\newcommand{\wheta}{\wh\eta}
\newcommand{\whgrc}{${\rm \widehat{g}}$lobal residue condition\xspace}
\newcommand{\whGrc}{${\rm \widehat{G}}$lobal residue condition\xspace}
\newcommand{\gkrc}{global $k$-residue condition\xspace}
\newcommand{\Gkrc}{Global $k$-residue condition\xspace}

\DeclareDocumentCommand{\Thick}{ O{(X,\bfz)} O{\epsilon}}{#1_{#2}}

%%%%%%%%%%%%%%%%%%%%%%%%%
%Real oriented blow up
\newcommand{\realbu}[1][X]{\overline{#1}^{\small{\RR}}}





%%%%%%%%%%%%%%%
\newcommand{\twkd}{twisted $k$-differential\xspace}
\newcommand{\twkds}{twisted\ $k$-differentials\xspace}
\newcommand*{\ptwkd}{prong-matched twisted $k$-differential\xspace}
\newcommand*{\ptwkds}{prong-matched twisted $k$-differentials\xspace}
\newcommand*{\Ptwkds}{Prong-matched twisted $k$-differentials\xspace}
\newcommand*{\mptwkd}{marked prong-matched twisted $k$-differential\xspace}
\newcommand*{\mptwkds}{marked prong-matched twisted $k$-differentials\xspace}

\newcommand*{\mskd}{multi-scale $k$-differential\xspace}
\newcommand*{\mskds}{multi-scale $k$-differentials\xspace}
\newcommand*{\auxkd}{model $k$-differential\xspace}
\newcommand*{\auxkds}{model $k$-differentials\xspace}

\newcommand*{\nmsd}{normalised multi-scale differential\xspace}
\newcommand*{\nmsds}{normalised multi-scale differentials\xspace}

\DeclareDocumentCommand{\LMSk}{ O{\mu} O{g}} {\Xi^{k}\overline\calM_{#2}(#1)}
\DeclareDocumentCommand{\LMSc}{ O{\wh\mu} O{\whg}} {\Xi\overline\calM_{#2}(#1)}
\DeclareDocumentCommand{\LMSkc}{ O{\wh\mu} O{\whg}} {\Xi^{\sim}\overline\calM_{#2}(#1)}


%musical annuli
\newcommand*{\Adoublesharp}{\mathcal{A}^{\musDoubleSharp}}
\newcommand*{\Asharp}{\mathcal{A}^{\musSharp}}
\newcommand*{\Adoubleflat}{\mathcal{A}^{\musDoubleFlat}}
\newcommand*{\Aflat}{\mathcal{A}^{\musFlat}}
\newcommand*{\Anatural}{\mathcal{A}^{\musNatural}}

\newcommand*{\AdoublesharpJ}{\mathcal{A}^{\musDoubleSharp,J}}
\newcommand*{\AsharpJ}{\mathcal{A}^{\musSharp,J}}
\newcommand*{\AdoubleflatJ}{\mathcal{A}^{\musDoubleFlat,J}}
\newcommand*{\AflatJ}{\mathcal{A}^{\musFlat,J}}
\newcommand*{\AnaturalJ}{\mathcal{A}^{\musNatural,J}}

\newcommand*{\AdoublesharpJp}{\mathcal{A}^{\musDoubleSharp,J'}}
\newcommand*{\AsharpJp}{\mathcal{A}^{\musSharp,J'}}
\newcommand*{\AdoubleflatJp}{\mathcal{A}^{\musDoubleFlat,J'}}
\newcommand*{\AflatJp}{\mathcal{A}^{\musFlat,J'}}
\newcommand*{\AnaturalJp}{\mathcal{A}^{\musNatural,J'}}


\newcommand*{\Fdoublesharp}{\mathcal{F}^{\musDoubleSharp}}
\newcommand*{\Fsharp}{\mathcal{F}^{\musSharp}}
\newcommand*{\Fdoubleflat}{\mathcal{F}^{\musDoubleFlat}}
\newcommand*{\Fflat}{\mathcal{F}^{\musFlat}}
\newcommand*{\Fnatural}{\mathcal{F}^{\musNatural}}

\newcommand*{\FdoublesharpJ}{\mathcal{F}^{\musDoubleSharp,J}}
\newcommand*{\FsharpJ}{\mathcal{F}^{\musSharp,J}}
\newcommand*{\FdoubleflatJ}{\mathcal{F}^{\musDoubleFlat,J}}
\newcommand*{\FflatJ}{\mathcal{F}^{\musFlat,J}}
\newcommand*{\FnaturalJ}{\mathcal{F}^{\musNatural,J}}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%obsolete abbrev

\newcommand{\IV}[1][\mu,\oGp]{{\mathcal I}^{\rm noGRC} ({#1})}
\newcommand{\IVGRC}[1][\mu,\oGp]{{\mathcal I}({#1})}

\newcommand{\TWGRC}[1][\oG]{TWGRC}
\newcommand{\TW}[1][\oG]{TW}

\newcommand{\pderiv}[1]{\frac{\partial}{\partial #1}}




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "PLUMB2"
%%% End:

